Improving generalization by mimicking the human visual diet

We present a new perspective on bridging the generalization gap between biological and computer vision -- mimicking the human visual diet. While computer vision models rely on internet-scraped datasets, humans learn from limited 3D scenes under diverse real-world transformations with objects in natural context. Our results demonstrate that incorporating variations and contextual cues ubiquitous in the human visual training data (visual diet) significantly improves generalization to real-world transformations such as lighting, viewpoint, and material changes. This improvement also extends to generalizing from synthetic to real-world data -- all models trained with a human-like visual diet outperform specialized architectures by large margins when tested on natural image data. These experiments are enabled by our two key contributions: a novel dataset capturing scene context and diverse real-world transformations to mimic the human visual diet, and a transformer model tailored to leverage these aspects of the human visual diet. All data and source code can be accessed at https://github.com/Spandan-Madan/human_visual_diet.

==> combined_figures_tex/fig_6_architecture.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\textwidth]{combined_figures/fig_6_architecture.pdf}
    \caption{\emph{Human Visual Diet enables substantially better generalization from synthetic to natural image data.}} 
    \label{fig:fig_6_architecture}
\end{figure}

==> figures_page.tex <==
\input{figures_tex/paradigm}
\input{figures_tex/architectures}
\input{figures_tex/geometric_accuracy}
\input{figures_tex/splits_accuracy}
\input{figures_tex/specialization}
\input{figures_tex/sscores}


==> figures_tex/MNIST-sscores.tex <==
\begin{figure*}[!b]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
     \includegraphics[width=0.255\linewidth]{figures/appendix/MNIST-sscores/MNIST-Position_units.pdf}
&
     \includegraphics[width=0.255\linewidth]{figures/appendix/MNIST-sscores/MNIST-Scale_units.pdf} 
&  \includegraphics[width=0.255\linewidth]{figures/appendix/MNIST-sscores/MNIST-Position_sscore_both.pdf} &  \includegraphics[width=0.255\linewidth]{figures/appendix/MNIST-sscores/MNIST-Scale_sscore_both.pdf}   \\
(a) & (b) & (c)& (d) \\
\end{tabular}
\caption{\emph{Neuron specialization in MNIST-Position and MNIST-Scale datasets}. (a) and (b) Percentage of neurons in the final convolutional layer of ResNet-18 that are specialized to category and viewpoint, for MNIST-Position and MNIST-Scale datasets, respectively. (c) and (d) Median of the specialization scores of neurons in the final convolutional layer of ResNet-18 \emph{Separate} and \emph{Shared} architectures, for category and viewpoint classification tasks, respectively.}
\label{fig:generalSation_datasets_tasks}
\end{figure*}

% geometric mean of category and pose prediction accuracy forSeparateandSharedarchitectures203with the ResNet18 backbone, 

==> figures_tex/MNIST_samples.tex <==
\begin{figure*}[!b]
\begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.25cm}}c}
\centering\includegraphics[width=0.48\linewidth]{figures/MNIST-Position.png}&
     \includegraphics[width=0.48\linewidth]{figures/MNIST-Scale.png}\\
     (a) MNIST-Position & (b) MNIST-Scale
\end{tabular}
 \caption{\emph{Combinations grids for MNIST-Position and MNIST-Scale.} Each row represents images from a category and each column from a viewpoint. (a) MNIST-Position was created by adding viewpoint in the form of position to images. For this, MNIST images were placed into one of nine positions in an empty three-by-three grid with equal probability. (b) MNIST-Scale was created by resizing images from MNIST to one of nine possible sizes, and then zero-padding.}
\label{fig:MNIST}
%  compared to after 4 blocks as in212the case of theSharedarchitecture as shown in Fig. 
%  The \textit{Separate} architecture, we train separate networks for each task. For the \textit{Shared} architecture, 
%  Networks trained separately for each task (\emph{Separate}) or trained for both with splits at different layers (\emph{Shared} and~\emph{Split-2}). ResNet18 with $4$ for block is displayed.}
\end{figure*}

==> figures_tex/accuracy_tasks.tex <==
\begin{figure*}[t!]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
     \includegraphics[width=0.255\linewidth]{figures/appendix/accuracy_tasks/MNIST-Position_accuracy_tasks.pdf}
&
     \includegraphics[width=0.255\linewidth]{figures/appendix/accuracy_tasks/MNIST-Scale_accuracy_tasks.pdf}
&  \includegraphics[width=0.255\linewidth]{figures/appendix/accuracy_tasks/iLab_accuracy_tasks.pdf} &  \includegraphics[width=0.255\linewidth]{figures/appendix/accuracy_tasks/Cars-City_accuracy_tasks.pdf}  \\
(a) & (b) & (c)& (d) \\
\end{tabular}
\caption{\emph{Generalization performance for category recognition and viewpoint estimation for \textit{Shared} and \textit{Separate} ResNet-18 as in-distribution combinations are increased for all datasets.} The category recognition accuracy and viewpoint estimation accuracy are reported along with confidence intervals (95\%) (a)~MNIST-Position dataset. (b)~MNIST-Scale dataset. (c)~iLab dataset. (d)~Biased-Cars dataset.}
\label{fig:accuracy_tasks}
\end{figure*}

% geometric mean of category and pose prediction accuracy forSeparateandSharedarchitectures203with the ResNet18 backbone, 

==> figures_tex/architectures.tex <==
\begin{figure*}[h!]
\begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
\centering\includegraphics[width=0.32\linewidth]{figures_tex/Shared_viewpoint.pdf}&
     \includegraphics[width=0.32\linewidth]{figures_tex/Separate_viewpoint.pdf}
& \includegraphics[width=0.32\linewidth]{figures_tex/Split-2_viewpoint.pdf}\\
% \small{Ford Thunderbird, Front} & \small{Mitsubishi Lancer, Side} & \small{Ford Thunderbird, Side} \\
% & (a) &\\[0.75em]
% \centering\includegraphics[width=0.32\linewidth]{figures/ILAB.png}
% & \includegraphics[width=0.32\linewidth]{figures/ilab_test_compositions.png}
% &
%      \includegraphics[width=0.32\linewidth]{figures/ilab_18_compositions.png}
%      \\
% \small{iLab-2M dataset}  &   \small{\emph{Unseen} Combinations (held-out)} & \small{ $50\%$ \emph{Seen} Combinations } \\
% (b) & (c) & (d)\\

\end{tabular}
 \caption{\emph{Architectures for Category Recognition and Viewpoint Estimation.} \textit{Shared}, \textit{Separate} and \textit{Split-2} architectures for ResNet-18. In the \textit{Shared} architecture, all layers until the last convolutional block are shared between tasks, followed by task specific fully connected branches. In the \textit{Separate} architecture, each task is trained in a separate network with no layer sharing. \textit{Split-2} presents a middle ground. These architectures are designed similarly for backbones other than ResNet-18.}
 \label{fig:architectures}
%  compared to after 4 blocks as in212the case of theSharedarchitecture as shown in Fig. 
%  The \textit{Separate} architecture, we train separate networks for each task. For the \textit{Shared} architecture, 
%  Networks trained separately for each task (\emph{Separate}) or trained for both with splits at different layers (\emph{Shared} and~\emph{Split-2}). ResNet18 with $4$ for block is displayed.
%\vspace{-0.5cm}
\end{figure*}

==> figures_tex/biased_cars_extrapolation_set.tex <==
\begin{figure*}[!b]
\centering\includegraphics[width=0.5\linewidth]{figures/controls/baised_cars_extrapolation_set.pdf}

 \caption{\emph{Generalization of \emph{Separate} architectures to OOD combinations as number of in-distribution combinations are increased while ensuring that viewpoints increasingly distant from the OOD set are added (Dissimilar Diversity).} To control that the increasing generalization performance as the data diversity increases is not due to closer viewpoint angles between In-distribution and OOD combinations, we created a dataset split where the In-distribution combinations start closest to the OOD combinations (in terms of viewpoint angle), and become increasingly distant. Thus, as In-distribution combinations are increased, the training data becomes increasingly dissimilar to the OOD combinations (test set). The results show that the performance on the OOD combinations still improves as data diversity increases. This experiment discards the hypothesis the increase in generalization performance is due to having closer viewpoint angles between the In-distribution and OOD combinations}.
\label{fig:baised_cars_extrapolation_set}
\end{figure*}
% \end{tabular}
% \begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}



==> figures_tex/cars-invariance.tex <==
\begin{figure*}[!t]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

\includegraphics[width=0.255\linewidth]{figures/appendix/Cars-invaraince/Cars-City_invariance_sscore_category_backbones.pdf}
&
\includegraphics[width=0.255\linewidth]{figures/appendix/Cars-invaraince/Cars-City_invariance_sscore_pose_backbones.pdf}
& 
\includegraphics[width=0.255\linewidth]{figures/appendix/Cars-invaraince/Cars-City_invariance_sscore_category.pdf}
& \includegraphics[width=0.255\linewidth]{figures/appendix/Cars-invaraince/Cars-City_invariance_sscore_pose.pdf}\\
(a) & (b) & (c)& (d) \\
\includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_category_backbones.pdf}
&
\includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_pose_backbones.pdf}
& 
\includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_category.pdf}
& \includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_pose.pdf}\\
(e) & (f) & (g)& (h) \\
\end{tabular}
\caption{\emph{Invariance and selectivity scores in the Biased-Cars dataset.} 
(a) and (b) Median of the invariance score among neurons in network architectures, other than ResNet-18, \emph{separate} and \emph{shared}, for category and viewpoint recognition tasks, respectively. Confidence intervals (95\%) are displayed in low opacity.
(c) and (d) Median of the invariance score among neurons in ResNet-18 \emph{Separate} and \emph{Shared} with splits made at different blocks of the network, for category and viewpoint recognition tasks, respectively. (e),(f),(g) and (h) Median of selectivity scores for architectures mentioned in experiments above.}
% \caption{\emph{Selectivity scores in the Biased-Cars dataset.} 
% (a) and (b) Median of the selectivity score among neurons in network architectures, other than ResNet-18, \emph{separate} and \emph{shared}, for category and viewpoint recognition tasks, respectively. Confidence intervals (95\%) are displayed in low opacity.
% (c) and (d) Median of the selectivity score among neurons in ResNet-18 \emph{Separate} and \emph{Shared} with splits made at different blocks of the network, for category and viewpoint recognition tasks, respectively. }
% \label{fig:specialization_scores_selectivity}
\label{fig:specialization_scores_invariance_and_selectivity}
\end{figure*}



==> figures_tex/cars-selectivity.tex <==
% \begin{figure*}[!t]
% \begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

% \includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_category_backbones.pdf}
% &
% \includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_pose_backbones.pdf}
% & 
% \includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_category.pdf}
% & \includegraphics[width=0.255\linewidth]{figures/appendix/Cars-selectivity/Cars-City_selectivity_sscore_pose.pdf}\\
% (a) & (b) & (c)& (d) \\
% \end{tabular}
% \caption{\emph{Selectivity scores in the Biased-Cars dataset.} 
% (a) and (b) Median of the selectivity score among neurons in network architectures, other than ResNet-18, \emph{separate} and \emph{shared}, for category and viewpoint recognition tasks, respectively. Confidence intervals (95\%) are displayed in low opacity.
% (c) and (d) Median of the selectivity score among neurons in ResNet-18 \emph{Separate} and \emph{Shared} with splits made at different blocks of the network, for category and viewpoint recognition tasks, respectively. }
% \label{fig:specialization_scores_selectivity}
% \end{figure*}



==> figures_tex/data_control.tex <==
% \begin{figure*}[!t]
% \begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
% \centering\includegraphics[width=0.5\linewidth]{figures/controls/data_control_biased_cars.pdf}&
%      \includegraphics[width=0.5\linewidth]{figures/controls/data_control_ilab.pdf}
% \end{tabular}
%  \caption{\emph{Generalization to OOD combinations as number of training images is varied.} For both iLab and Biased-Cars dataset, \textit{Separate} architecture outperforms the \textit{Shared} architecture trained with the same number of images.}
%  \label{fig:data_control}
% \end{figure*}

==> figures_tex/gcnns.tex <==
% \begin{figure*}[!t]
% \begin{tabular}{@{\hspace{0.0cm}}c@{\hspace{0.1cm}}c}
% \centering\includegraphics[width=0.5\linewidth]{figures/rebuttal_figures/spherical_cnns.pdf}&
%      \includegraphics[width=0.5\linewidth]{figures/rebuttal_figures/icosahedral_cnns.pdf}
% \end{tabular}
%  \caption{\emph{Generalization performance for different group equivariant architectures as in-distribution combinations are increased for MNIST-Rotation dataset.} The geometric mean of category recognition accuracy and viewpoint estimation accuracy is reported for OOD combinations as the number  of in-distribution combinations  is increased. (a) Accuracy of \textit{Separate} and \textit{Shared} architectures using a Spherical CNN~\citep{cohen2018spherical} as backbone, (b) Accuracy using an Icosahedral CNN~\citep{cohen2019gauge} as backbone.}
% \label{fig:gcnns}
% \end{figure*}

==> figures_tex/generalization_to_scannet.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/generalization_to_scannet.pdf}
    \caption{\textbf{Human visual diet enables substantially better generalization to real world ScanNet images}. We report the capability of models to generalize from synthetic \textit{HVD} images to the natural image ScanNet dataset. CTCNet leverages human like visual-diet and is able to outperform both standard architectures, and specialized domain generalization approaches.}
    \label{fig:generalization_to_scannet}
\end{figure*}

==> figures_tex/geometric_accuracy.tex <==
\begin{figure*}[h!]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
     \includegraphics[width=0.255\linewidth]{figures/geom_accuracy/MNIST-Position_accuracy.pdf}
&
     \includegraphics[width=0.255\linewidth]{figures/geom_accuracy/MNIST-Scale_accuracy.pdf}
&  \includegraphics[width=0.255\linewidth]{figures/geom_accuracy/iLab_accuracy.pdf} &  \includegraphics[width=0.255\linewidth]{figures/geom_accuracy/Cars-City_accuracy.pdf} \\
(a) & (b) & (c)& (d) \\
\end{tabular}
\caption{\emph{Generalization performance for \textit{Shared} and \textit{Separate} ResNet-18 as in-distribution combinations are increased for all datasets.} The geometric mean of category recognition accuracy and viewpoint estimation accuracy is reported along with confidence intervals (95\%) (a)~MNIST-Position dataset. (b)~MNIST-Scale dataset. (c)~iLab dataset. (d)~Biased-Cars dataset.}
\label{fig:generalSation_datasets}
\end{figure*}

% geometric mean of category and pose prediction accuracy forSeparateandSharedarchitectures203with the ResNet18 backbone, 

==> figures_tex/iLab-sscores.tex <==
\begin{figure*}[!h]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

\includegraphics[width=0.255\linewidth]{figures/appendix/iLab-sscores/iLab_sscore_category_backbones.pdf}
&
\includegraphics[width=0.255\linewidth]{figures/appendix/iLab-sscores/iLab_sscore_pose_backbones.pdf}
& 
\includegraphics[width=0.255\linewidth]{figures/appendix/iLab-sscores/iLab_sscore_category.pdf}
& \includegraphics[width=0.255\linewidth]{figures/appendix/iLab-sscores/iLab_sscore_pose.pdf}\\
(a) & (b) & (c)& (d) \\
\end{tabular}
\caption{\emph{Neuron specialization (selectivity to category and invariance to viewpoint, and vice versa) in the iLab dataset.} 
(a) and (b) Median of the specialization score among neurons ($\Gamma^k$) in network architectures, other than ResNet-18, \emph{separate} and \emph{shared}, for category and viewpoint classification tasks, respectively.  Confidence intervals (95\%) are displayed in low opacity.
(c) and (d) Median of the specialization score among neurons in ResNet-18 \emph{Separate} and \emph{Shared} with splits made at different blocks of the network, for category and viewpoint classification tasks, respectively. Similar results for the \textit{Biased-Cars} dataset are provided in the main paper.}
\label{fig:specialization_scores_iLab}
\end{figure*}



==> figures_tex/layers.tex <==
\begin{figure*}[!t]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

\includegraphics[width=0.255\linewidth]{figures/appendix/layers/iLab_sscore_layer_category.pdf}
&
\includegraphics[width=0.255\linewidth]{figures/appendix/layers/iLab_sscore_layer_pose.pdf}
& 
\includegraphics[width=0.255\linewidth]{figures/appendix/layers/Cars-City_sscore_layer_category.pdf}
& \includegraphics[width=0.255\linewidth]{figures/appendix/layers/Cars-City_sscore_layer_pose.pdf}\\
(a) & (b) & (c)& (d) \\
\end{tabular}
\caption{\emph{Specialization Score Per Layer for $30$ \emph{seen} category-viewpoint Combinations for iLab, and $20$ \emph{seen} category-viewpoint Combinations for the \textit{Biased-Cars} dataset.} 
(a) and (b) Median of the specialization score among neurons in ResNet-18 \emph{Separate} and \emph{Shared} with splits made at different blocks of the network, for category and viewpoint classification tasks, respectively. (c) and (d) Same as (a) and (b) for \emph{Biased-Cars} dataset. }
\label{fig:specialization_scores_layers}
\end{figure*}



==> figures_tex/paradigm.tex <==
\newpage
\begin{figure*}[h!]
\begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
\centering\includegraphics[width=0.32\linewidth]{figures/thunderbird_front_large.png}&
     \includegraphics[width=0.32\linewidth]{figures/evo_side.png}
& \includegraphics[width=0.32\linewidth]{figures/thunderbird_side_2.png}\\
\small{Ford Thunderbird, Front} & \small{Mitsubishi Lancer, Side} & \small{Ford Thunderbird, Side} \\
& (a) &\\[0.75em]
\centering\includegraphics[width=0.32\linewidth]{figures/ILAB.png}
& \includegraphics[width=0.32\linewidth]{figures/ilab_test_compositions.png}
&
     \includegraphics[width=0.32\linewidth]{figures/ilab_18_compositions.png}
     \\
\small{iLab-2M dataset}  &   \small{OOD Combinations (held-out)} & \small{ $50\%$ in-distribution Combinations } \\
(b) & (c) & (d)\\

\end{tabular}
\caption{\emph{Category-Viewpoint datasets.} (a) Our new \textit{Biased-Cars} dataset: Can a network shown only the Ford Thunderbird from front and the Mitsubishi Lancer from side generalize to classify the category and viewpoint for a Thunderbird seen from the side? (b) iLab-2M dataset~\citep{borji2016ilab}: Each cell represents a unique category-viewpoint combination (categories vary between rows, viewpoints between columns) with multiple object instances per category and backgrounds. (c) Held-out test set of category-viewpoint combinations. Same held-out test set is used to evaluate networks trained with different number of in-distribution combinations. (d) Biased training set with $50\%$ of category-viewpoint combinations. Number of categories and viewpoints selected is always equal. }
\label{multi_attribute_datasets}
%\vspace{-0.5cm}
\end{figure*}

==> figures_tex/specialization.tex <==

\begin{figure*}[h!]
\begin{tabular}{@{\hspace{0.2cm}}c@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c}
\centering
 \multirow{1}{*}{
\begin{tabular}{c}
 \vspace*{-3.8cm}\\
\includegraphics[width=0.42\linewidth]{figures/fig1.pdf}\\
(a)
\end{tabular}
}
&  \includegraphics[width=0.25\linewidth]{figures/specialization/iLab_units.pdf} &  \includegraphics[width=0.25\linewidth]{figures/specialization/Cars-City_units.pdf}
 \\
 & (b) & (c) \\
\end{tabular}
\caption{\emph{Specialization to category recognition and viewpoint estimation.}  (a) Prototypical \emph{activation grids} for different types of selective and invariant neurons. (b) and (c) Percentage of neurons after ResNet-18 block-4 that are  specialized to category and viewpoint, for iLab and Biased-Cars datasets, respectively. ResNet-18 \emph{Separate} and \emph{Shared} networks are evaluated; for \emph{Separate}, only the task-relevant neurons for each branch are displayed.  \vspace{-0.4cm}}
\label{fig:specialization}
\end{figure*}



==> figures_tex/splits_accuracy.tex <==
\begin{figure*}[h!]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
\includegraphics[width=0.255\linewidth]{figures/splits/iLab_splits_backbones_accuracy.pdf} &  \includegraphics[width=0.255\linewidth]{figures/splits/Cars-City_backbones_accuracy.pdf}  
&
\includegraphics[width=0.255\linewidth]{figures/splits/iLab_splits_accuracy.pdf}
&
     \includegraphics[width=0.255\linewidth]{figures/splits/Cars-City_splits_accuracy.pdf}
 \\
(a) & (b) & (c)& (d) \\
\end{tabular}
\caption{\emph{Generalization performance for different architectures and backbones as in-distribution combinations are increased for iLab and Biased-Cars datasets.} The geometric mean between  category recognition accuracy and viewpoint recognition accuracy is reported for OOD combinations as number of in-distribution combinations is increased. (a) and (b) Accuracy of  \emph{Separate} and \emph{Shared} for backbones other than ResNet-18, for iLab and Biased-Cars datasets, respectively. (c) and (d) Accuracy of ResNet-18 \emph{Separate}, \emph{Shared} and different \textit{Split} architectures made by splitting at different blocks of the network, for iLab and Biased-Cars datasets, respectively. }
\label{fig:controls}
\end{figure*}



% Comparison of networks trained separately for each task (\emph{Separate}) or trained for both (\emph{Shared}).

==> figures_tex/sscores.tex <==
\begin{figure*}[h!]
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}

\includegraphics[width=0.255\linewidth]{figures/sscores/Cars-City_sscore_category_backbones.pdf}
&
\includegraphics[width=0.255\linewidth]{figures/sscores/Cars-City_sscore_pose_backbones.pdf}
& 
\includegraphics[width=0.255\linewidth]{figures/sscores/Cars-City_sscore_category.pdf}
& \includegraphics[width=0.255\linewidth]{figures/sscores/Cars-City_sscore_pose.pdf}\\
(a) & (b) & (c)& (d) %\vspace{-0.2cm}
\end{tabular}
\caption{\emph{Neuron specialization (selectivity to category and invariance to viewpoint, and vice versa) in the Biased-Cars dataset.} (a) and (b) Median specialization score of neurons ($\Gamma^k$) in \emph{Separate} and \emph{Shared} architectures for category and viewpoint classification tasks respectively, for backbones other than ResNet-18. Confidence intervals (95\%) displayed in low opacity.(c) and (d) Median specialization score of neurons in ResNet-18 \emph{Separate} and \emph{Shared} architectures with splits made at different blocks of the network, for category and viewpoint classification tasks respectively. }%\vspace{-0.4cm}}

\label{fig:specialization_scores}
\end{figure*}



==> figures_tex/training_protocol.tex <==
\begin{figure*}[!t]
\centering
\begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
\includegraphics[width=0.35\linewidth]{figures/rebuttal_figures/training_protocol_ilab.pdf}&
     \includegraphics[width=0.35\linewidth]{figures/rebuttal_figures/training_protocol_biased_cars.pdf} \\
     \multicolumn{2}{c}{(a)}\\
     \includegraphics[width=0.35\linewidth]{figures/rebuttal_figures/uiuc_3d.pdf}&
     \includegraphics[width=0.35\linewidth]{figures/rebuttal_figures/mnist_rotation.pdf} \\
     \multicolumn{2}{c}{(b)} \\
     \includegraphics[width=0.35\linewidth]{figures/rebuttal_figures/spherical_cnns.pdf}&
     \includegraphics[width=0.35\linewidth]{figures/rebuttal_figures/icosahedral_cnns.pdf}\\
     \multicolumn{2}{c}{(c)}
\end{tabular}
\caption{\emph{Additional Results.} The geometric mean of category recognition accuracy and viewpoint estimation accuracy is reported for OOD combinations as the number  of in-distribution combinations  is increased. (a) Generalization performance for additional training protocols, besides Separate and Shared protocols, for the ResNet-18 backbone.  For these, we start by training the shared network on only one task first, \ie \textit{Viewpoint  first} or \textit{Category first}. We then train the second task starting from these learned features from the first task. We present their comparison with our \textit{Shared} and \textit{Separate} training protocols presented in the main paper. We report accuracy for the iLab dataset, and for the Biased-Cars dataset. (b) Generalization performance for additional datasets for ResNet-18 backbone.  We report the accuracy for the UIUC 3D dataset, and for the MNIST-Rotation dataset. Due to the small size of the UIUC dataset there is poor generalization - there are only 1700 train set for 37.5\% in-distribution combinations (which is kept constant as the number of in-distribution combinations increases). This leads to lesser generalization, but our findings still hold true. (c) Generalization performance for group equivariant architectures (Spherical CNN~\citep{cohen2018spherical} and  Icosahedral CNN~\citep{cohen2019gauge}) for MNIST-Rotation dataset. }


% \caption{\emph{Generalization performance for additional datasets for ResNet-18 backbone.} The geometric mean of category recognition accuracy and viewpoint estimation accuracy is reported for OOD combinations as the number  of in-distribution combinations is increased. (a) Accuracy for the UIUC 3D dataset, (b) Accuracy for the MNIST-Rotation dataset. Due to the small size of the UIUC dataset there is poor generalization - there are only 1700 train set for 37.5\% in-distribution combinations (which is kept constant as the number of in-distribution combinations increases). This leads to lesser generalization, but our findings still hold true - (1) Increasing in-distribution combinations improves performance on OOD data, and (2) \textit{Separate} architectures outperform \textit{Shared} ones on OOD combinations.}
% \label{fig:uiuc_3d_mnist_rotation}

%  \caption{\emph{Generalization performance for different group equivariant architectures as in-distribution combinations are increased for MNIST-Rotation dataset.} The geometric mean of category recognition accuracy and viewpoint estimation accuracy is reported for OOD combinations as the number  of in-distribution combinations  is increased. (a) Accuracy of \textit{Separate} and \textit{Shared} architectures using a Spherical CNN~\citep{cohen2018spherical} as backbone, (b) Accuracy using an Icosahedral CNN~\citep{cohen2019gauge} as backbone.}
% \label{fig:gcnns}
\label{fig:additional_results}
\end{figure*}

==> figures_tex/uiuc_3d_mnist_rotation.tex <==
% \begin{figure*}[!t]
% \begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
% \centering\includegraphics[width=0.5\linewidth]{figures/rebuttal_figures/uiuc_3d.pdf}&
%      \includegraphics[width=0.5\linewidth]{figures/rebuttal_figures/mnist_rotation.pdf}
% \end{tabular}
% \caption{\emph{Generalization performance for additional datasets for ResNet-18 backbone.} The geometric mean of category recognition accuracy and viewpoint estimation accuracy is reported for OOD combinations as the number  of in-distribution combinations is increased. (a) Accuracy for the UIUC 3D dataset, (b) Accuracy for the MNIST-Rotation dataset. Due to the small size of the UIUC dataset there is poor generalization - there are only 1700 train set for 37.5\% in-distribution combinations (which is kept constant as the number of in-distribution combinations increases). This leads to lesser generalization, but our findings still hold true - (1) Increasing in-distribution combinations improves performance on OOD data, and (2) \textit{Separate} architectures outperform \textit{Shared} ones on OOD combinations.}
% \label{fig:uiuc_3d_mnist_rotation}
% \end{figure*}

==> figures_tex/width_control.tex <==
\begin{figure*}[!t]
% \centering\begin{tabular}{@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c@{\hspace{0.1cm}}c}
\centering
\begin{tabular}{@{\hspace{-0.cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c@{\hspace{-0.1cm}}c}
\includegraphics[width=0.255\linewidth]{figures/controls/ResNet18_widths.pdf}&
\includegraphics[width=0.255\linewidth]{figures/controls/backbones_width.pdf}&
\includegraphics[width=0.255\linewidth]{figures/controls/data_control_biased_cars.pdf}&
\includegraphics[width=0.255\linewidth]{figures/controls/data_control_ilab.pdf}\\
{(a)} & {(b)} & {(c)} & {(d)} \\
\multicolumn{2}{c}{
\includegraphics[width=0.4\linewidth]{figures/rebuttal_cars}}&
\multicolumn{2}{c}{\includegraphics[width=0.4\linewidth]{figures/controls/rebuttal_2.pdf}}\\
\multicolumn{2}{c}{(e)}&
\multicolumn{2}{c}{(f)}\\
\multicolumn{2}{c}{
\includegraphics[width=0.4\linewidth]{figures/rebuttal_poses}}&
\multicolumn{2}{c}{\includegraphics[width=0.4\linewidth]{figures/controls/rebuttal_3.pdf}}\\
\multicolumn{2}{c}{(g)}&
\multicolumn{2}{c}{(h)}\\
% \includegraphics[width=0.22\linewidth]{figures/rebuttal_poses} &  
% \includegraphics[width=0.22\linewidth]{figures/controls/rebuttal_3.pdf}\\
\vspace{-2ex}
\end{tabular}
 \caption{\emph{Additional controls on generalization to OOD combinations.} (a), (b) Impact of varying number of neurons per layer for (a) the ResNet-18 backbone  and (b) other backbones. \textit{Separate} architectures substantially outperform \textit{Shared} architectures across a range of widths, \ie number of neurons per layer. The \textit{Separate} architecture contains double the parameters as the \textit{Shared} architecture, as there is no weight sharing in the \textit{Separate} case. Variants of these architectures are created by increasing or decreasing the neurons in each layer by a factor of 2 at a time. Even at one-eighth the number of neurons, the \textit{Separate One Fourth} architecture generalizes much better to OOD combinations as compared to the \textit{Shared Four Times} architecture. (c), (d) Impact as number of training images is varied. For both iLab and Biased-Cars dataset, \textit{Separate} architecture outperforms the \textit{Shared} architecture trained with the same number of images. (e), (f), (g) and (h) Controlling category and viewpoint separately. (e) Images of 4 new car categories, (f) Viewpoint classification accuracy for the 4 new car categories, (g) Images of new viewpoints, (h) Car category recognition accuracy for the new viewpoints.}
\label{fig:additional_controls}
%  \label{fig:width_control}
%  \caption{\emph{Generalization to OOD combinations as number of training images is varied.} For both iLab and Biased-Cars dataset, \textit{Separate} architecture outperforms the \textit{Shared} architecture trained with the same number of images.}
%  \label{fig:data_control}
 
%  \caption{\emph{Controlling category and viewpoint separately.}
%  (a) Images of 4 new car categories, (b) Viewpoint classification accuracy for the 4 new car categories, (c) Images of new viewpoints, (d) Car category recognition accuracy for the new viewpoints.}
%  \label{fig:rebuttal_exp}

\end{figure*}

==> how.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\textwidth]{combined_figures/fig_1_overview.pdf}
    \caption{\emph{Mimicking and exploiting the human visual diet.}} 
    \label{fig:fig_1_overview}
\end{figure}

==> rebuttal_1.tex <==

% \begin{comment}
% \documentclass{article}
% \usepackage{iclr2021_conference,times}
% % \usepackage{titling}

% \newcommand*{\eg}{\emph{e.g.,~}}
% \newcommand*{\ie}{\emph{ie.,~}}
% \newcommand*{\etal}{\emph{et al.~}}
% \newcommand*{\etc}{\emph{etc.}}

% \iclrfinalcopy

% \title{Response to concerns raised by Reviewer 1}
% \author{}
% \begin{document}
% \maketitle
% \vspace{-2cm}
% % \section{Comments for the esteemed Reviewer 1}

% \end{comment}
\newpage
 \setcounter{section}{0}

\section*{Response to concerns raised by Reviewer 1}
We thank the reviewer for their detailed comments. The crux of the review is that our findings are---(1) already known or obvious (non-novel), and (2) missing actionable insights which can be useful to practitioners. However, we believe this sentiment stems in part from our work being misunderstood, as there are several factual errors in the review. Below, we clarify these misunderstandings, followed by elucidating the novelty and impact of our results. 


We have also updated our manuscript to clarify these misunderstandings. This includes: (1) a slight change in the terminology (seen combinations to in-distribution combinations, and unseen combinations to OOD combinations), (2) adding additional details to the figures (all figures mention that the dataset size is fixed), (3) re-writing the titles, abstract, introduction, results and conclusions to emphasize our three findings and their novelty and significance. 



\section{Clarifying factual errors in the review}

\textit{\textbf{R1: ``Networks generalize better as they are fed more training data''}}\\
\textbf{Networks are never trained with more data:} All networks are fed the same amount of data in order to assess the impact of data diversity. As the number of category-viewpoint combinations (data diversity) shown during training increases, images per combination is reduced to keep the number of images used for training constant. 
\\\\

\textit{\textbf{R1: ``Results on synthetic datasets may not be applicable to real data''}}\\
\textbf{All findings reported on six datasets, including two real image datasets:} We confirm that our results extend to real data through experiments on iLab-2M and UIUC 3D datasets.
\\\\

\textit{\textbf{R1: ``Two networks surely will have perfect performance for each task''}}\\
\textbf{Multi-Task Learning literature reports otherwise:} \textit{Shared} architectures (learning shared representations across tasks) can significantly outperform \textit{Separate} ones, as shown in \cite{caruana1997multitask, ruder2017overview, zhang2018overview, zhang2021survey}. This behaviour is in fact the fundamental principle underlying Multi-Task Learning.
\\\\

\textit{\textbf{R1: ``Shared feature will drop performance no matter on unseen or seen''}}\\
\textbf{Different impact of sharing features on in-distribution (seen) and OOD (unseen) combination:} A striking finding that emerged from our analysis is the contrast in the trends of the in-distribution (seen) and OOD (unseen) performance. Fig.~\ref{fig:generalSation_datasets} reports that sharing features leads to a marginal improvement in performance on in-distribution (seen) combinations, similar to the multi-task learning literature cited above. Shared features drop performance only when tested on OOD (unseen) combinations.
\\\\

% \textit{\textbf{R1: ``Tons of work evaluate viewpoint and category for CNNs''}}\\
% \textbf{Single vs Multi-Task Learning:} Existing works perform single task prediction. For eg., category classification across unseen viewpoints [X,Y] predicts only category treating viewpoint as a nuisance parameter. We predict both parameters (Multi-Task Learning) and evaluate generalization to unseen combinations (out-of-distribution). Not just viewpoints, categories too are unseen. Thus, we study generalization out of distribution for multiple task prediction.


\textit{\textbf{R1: ``[The neuron's] selectivity to category or viewpoint is obvious to know, even without doing any measurement.''}}\\
The framework of selectivity and invariance does not extend to the multi-task problem of simultaneous category and viewpoint classification. We introduce the specialization score, which extends these to ideas to multi-task learning and measures specialization.


\section{Novelty and Applications of our findings}
We focus on understanding \emph{when} and \emph{how} CNNs may generalize to OOD category-viewpoint combinations. We have rewritten the paper to clarify our discoveries. In the following, we present them along with the applications.

    

\subsection{Data diversity significantly impacts OOD performance}


\noindent\textbf{Summary}: We investigate the role of data diversity by varying the number of in-distribution category-viewpoint combinations, keeping dataset size constant. We find that data diversity matters significantly. For a constant dataset size, increasing data diversity makes the task more challenging, as reflected in the deteriorating in-distribution performance. Yet, increasing data diversity substantially improves performance on OOD combinations. 

\noindent \textbf{Evidence and Novelty}:
Fig.~\ref{fig:generalSation_datasets} presents the geometric mean of category and viewpoint classification accuracy for \textit{Separate} and \textit{Shared} architectures with the ResNet-18 backbone, for all datasets. These experiments were repeated three times, and here we present the mean performance with confidence intervals. 
For fixed dataset size, increasing in-distribution combinations makes the task more challenging as images with each category and viewpoint become more diverse, leading to some drop in accuracy on in-distribution combinations. In contrast, both architectures show a significant improvement of their performance on images from OOD combinations, as data diversity increases. We ensured that this result can not be attributed to having closer viewpoint angles between in-distribution and OOD combinations as data diversity is increased (supplement~\ref{sec:suplSimilarity}). CNNs do not theoretically guarantee viewpoint invariance~\citep{poggio2016visual}, but our result provides reassurance that CNNs can become robust to OOD category-viewpoint combinations as long as they are shown enough diversity during training. Taken together, these results suggest an inherent trade-off between getting better on in-distribution combinations and extrapolating to OOD combinations, which is impacted by training data diversity. Also, these results add to a growing body of works investigating the trade-offs inherent to multi-task learning~\citep{standley2019tasks, shin2018pixels}.


Even though the geometric mean of category and viewpoint classification increases consistently with increased in-distribution combinations, individual accuracy for these tasks does not always increase consistently (see supplement~\ref{sec:suplSeparateAcc}). We attribute this to the randomness in the selection of in-distribution and OOD combinations. Furthermore, the relative accuracy of the two tasks varies depending on the dataset, and no task is consistently harder than the other across all datasets.


\textbf{For practitioners - Guidelines for building datasets that enable OOD generalization:} Our findings show that if practitioners expect out-of-distribution images in deployment, they should try to collect as diverse a dataset as possible, instead of only worrying about dataset size. In fact, it may not even matter if the added images are more dissimilar to the test set, as we have shown---just add more diversity for better out-of-distribution performance.




% rule of thumb of collecting as many new images as possible (for eg., through internet scraping). Concretely, Fig.X shows that less data can significantly outperform more data if diversity is high when tested out of distribution. Furthermore, Fig.Y shows that even if dissimilar, just add more data during training for better generalization. These findings provide useful guidelines for computer vision applications where out of distribution behaviour is important.
\subsection{Separate architectures outperform shared ones on OOD combinations}

\noindent \textbf{Summary:} We also analyze the performance of different architectures in the multi-task setting of simultaneous category and viewpoint classification,~\ie learning category and viewpoint in \emph{Shared} or in \emph{Separate} (no layers shared) architectures.
     Our results reveal that \emph{Separate} architectures generalize substantially better to OOD combinations compared to \emph{Shared} architectures. Also, this trend is in stark contrast with the trend for in-distribution combinations, where \emph{Shared} architectures perform marginally better. Thus, the belief that \emph{Shared} architectures outperform \emph{Separate} ones when tasks are synergistic should be revisited~\citep{caruana1997multitask}, as their relative performance strongly depends on whether the test sample is in-distribution or OOD.
    
     
     
\noindent \textbf{Evidence and Novelty:} A striking finding that emerged from our analysis is the contrast in the trends of the in-distribution and OOD performance. While both architectures perform well on new images from in-distribution combinations, \textit{Separate} architectures outperform \textit{Shared} ones by a very large margin on OOD combinations. For the ResNet-18 backbone, this result can be seen consistently across all $4$ datasets as shown in Fig.~\ref{fig:generalSation_datasets}. Supplement~\ref{sec:suplSeparateAcc} shows that \emph{Separate} also outperforms \emph{Shared} for category and viewpoint classification individually. Note that previous works have shown that \textit{Shared} architectures are superior for synergistic tasks, as networks can share features among tasks. These works test on the same combinations as seen during training (in-distribution), and when we do so, we also observe that \textit{Shared} architectures perform same or slightly better than \textit{Separate} ones (Fig.~\ref{fig:generalSation_datasets} dashed lines). Thus, our results reveal that the relative performance between \textit{Shared} and \textit{Separate} depends not only on the synergy between tasks, but also whether the evaluation is in-distribution or OOD. 


We extended our analysis to \emph{Separate} and \emph{Shared} architectures with different backbones, namely ResNeXt~\citep{xie2017aggregated}, WideResNet~\citep{zagoruyko2016wide}, Inception v3~\citep{szegedy2016rethinking} and the DenseNet~\citep{huang2017densely}, as shown in Fig.~\ref{fig:controls}a and b. As can be seen, \emph{Separate} architectures outperform \emph{Shared} ones by a large margin for all backbones, which confirms that this result is not backbone specific. Investigating further, we experiment with \emph{Split} architectures, and as can be seen in Fig.~\ref{fig:controls}c and d, there is a consistent, gradual dip in the performance as we move from the \textit{Separate} to the \textit{Shared} architectures. Thus, generalization to OOD category-viewpoint combinations is best achieved by learning both tasks separately, with a consistent decrease in generalization as more parameter sharing is enforced.

To make sure that \textit{Separate} architectures do not perform better due to the added number of neurons, we made the \textit{Shared-Wide} architecture by doubling the neurons in each layer of the \textit{Shared} ResNet-18 network. As Fig.~\ref{fig:controls}c and d show, this architecture performs very similarly to the \textit{Shared} one (see additional results in ~\ref{app:NumberNeurons}). This is in accordance with previous results that show that modern CNNs may improve in performance as the width is increased but to a limited extent~\citep{nakkiran2019deep,casper2019removable}. 

In the supplement, we provide a number of additional controls that support the generality of our results. Concretely, we show results for different number of training images (supplement~\ref{app:NumberTraining}), viewpoint estimation for 4 new car models and category prediction for new viewpoints (supplement ~\ref{app:DifferentBias}), and the order in which category and viewpoint are learned (supplement ~\ref{app:TaskOrder}). We also present results on additional datasets (supplement~\ref{app:AdditionalDatasets}) and architectures (supplement~\ref{app:AdditionalArch}).

\textbf{For practitioners - Guidelines for architecture design:} The combination of object recognition and viewpoint estimation is essential for effective visual understanding, and our work shows that the choice of architecture should depend on whether the practitioner expects more in-distribution or out-of-distribution samples in deployment. If the practitioner expects more out-of-distribution samples in deployment, \textit{Separate} architectures should be used in deployment. Otherwise, \textit{Shared} ones should be chosen. 
% \subsection{Separate architectures outperform Shared ones on unseen combinations}
% Review states ``two networks...surely will have perfect performance for each task''. However, existing work on multi-task learning shows this is not the case---Shared architecture are superior as they can share features among tasks. Our results confirm the same for Seen combinations. The novelty of our work is that unlike past work we also evaluate multi-task networks on Unseen combinations. Contrary to expectation and past literature, we show that only changes on Unseen combinations Separate architectures outperform Shared ones.
\subsection{Neural Specialization facilitates generalization to OOD combinations}


\noindent \textbf{Summary:} Existing works suggest that OOD generalization is facilitated by selective and invariant representations~\citep{giles1987learning,riesenhuber1998just,goodfellow2009measuring,achille2018emergence}. However, this has not been previously demonstrated for deep learning, and does not extend to simultaneous category and viewpoint classification. To address this, we propose the neural mechanism of specialization---the emergence of two types of neurons, one driving OOD generalization for category, and the other for viewpoint. This corresponds to neurons selective to a category and invariant to viewpoint, and vice versa. We show that CNN generalization behavior trends correlate with the degree of specialization of the neurons.
    
    
    

\noindent \textbf{Evidence and Novelty:}    We first investigate the emergence of category and viewpoint neurons in the final convolutional layer of the networks. Fig.~\ref{fig:specialization}b and c show the percentage of neurons of each type in \emph{Shared} and \emph{Separate} architectures as in-distribution combinations are increased. As can be seen, all neurons in the category and viewpoint branches of the \textit{Separate} architecture become specialized to category and viewpoint respectively. But in the \textit{Shared} case, as the network is expected to simultaneously learn both tasks, both kinds of neurons emerge at a ratio of about $50\%$. We found that this ratio depends on the relative weight of loss terms for the two tasks. When using a different weight from the optimal in terms of maximum geometric mean accuracy, the $50\%$ ratio of specialized neuron becomes unbalanced. For a small number of in-distribution combinations, the ratio of specialized neurons may also be impacted by the relative difficulty of two tasks, with more neurons becoming specialized for the easier task (see supplement~\ref{app:SpecializationAdditionalDatasets}).

In Fig.~\ref{fig:specialization_scores} we present the median of specialization scores across neurons,~\ie the median of $\Gamma^k$, in the final convolutional layer for \emph{Shared}, \emph{Split}, and \emph{Separate} architectures across multiple backbones in \textit{Biased-Cars} dataset (see supplement~\ref{app:specializationiLab} for results in other datasets). These results are presented separately for the category and viewpoint neurons. We show that as in-distribution combinations increase, there is a steady increase in the specialization score for both category and viewpoint neurons, suggesting specialization. These trends mirror the generalization trends, which suggests that specialization facilitates OOD generalization. Invariance and selectivity scores are reported separately in supplement ~\ref{app:InvarianceAndSelectivity}. We also show that specialization builds up across layers (supplement~\ref{app:SpecializationBuilds}) as expected~\citep{goodfellow2009measuring,poggio2016visual}.


Finaly, Fig.~\ref{fig:specialization_scores} shows that \textit{Separate} architectures facilitate  specialization, while the \emph{Shared} architecture makes it harder for the neurons to specialize (lower specialization scores). This might be because unlike the \emph{Shared} architecture, the branches of the \textit{Separate} architecture are not forced to preserve features relevant to both tasks. Each branch can develop features which are selective to only one task, and invariant to the other. This may facilitate an increase in specialization and thus enable better performance on OOD combinations. Even though the \emph{Shared} architecture tries to split into two specialized parts, this specialization is much stronger in the \textit{Separate} architecture due to already having separate branches.



% The proposed \textit{Specialization score} is an exntension of selectivity and invariance, and correlates strongly with out-of-distribution performance. Our findings show that Separate architectures enable Specialization, which leads to better generalization out-of-distribution.

% \textbf{Novelty:} Selective and Invariant representations have proved to be useful frameworks for studying generalization in single task prediction. However, these does not extend to multi-task learning. Specialization extends on the these ideas to provide a framework for studying generalization behaviour in Multi-Task prediction. 

\textbf{For practitioners - Improving out-of-distribution behavior of models:} In applications where out-of-distribution performance is crucial, specialization score can be used as a proxy objective function in the form of a loss function, or as a performance metric for model selection.
% \section{Concern 2: Applications/Actionable insights from results}
% \subsection{Guidelines for data collection to enable out-of-distribution generalization}
% Practitioners routinely collect new, custom datasets for varied applications. The practitioner's rule of thumb is to collect as many new images as possible, often through large-scale internet scraping. However, our work shows that future datasets must be cognizant of data diversity even more. Concretely, Fig.X shows that less data can significantly outperform more data if diversity is high when tested out of distribution. Furthermore, Fig.Y shows that even if dissimilar, just add more data during training for better generalization. These findings provide useful guidelines for computer vision applications where out of distribution behaviour is important.

% \subsection{Architecture design for better generalization}


% \subsection{Specialization as a diagnostic tool}


% \bibliography{library}
% \bibliographystyle{iclr2021_conference}

% \end{document}


\section*{Response to concerns raised by Reviewer 2}

We thank the reviewer for the in-depth review, and for their insightful comments and suggestions. We appreciate that the reviewer mentions: ``I think the submission is a novel and strong contribution towards understanding the relationship between viewpoint and category classification accuracy of networks and dataset diversity/network architecture''. 

We have updated our manuscript to incorporate the reviewer's suggestions, and to answer the questions raised by them. Below, we present these updated parts of our manuscript.

% In the following, we address the reviewer's concerns:

\textbf{R2: Explain more detail about the trade-off between viewpoint and category classification.} 

In supplement~\ref{sec:suplSeparateAcc}, cited in the "When" section of the main paper, we have added the following discussion: 

The relative accuracy of the two tasks varies depending on the dataset, and no task is consistently harder than the other across all datasets. For instance, viewpoint classification is easier for MNIST-Position, while it is significantly hard for MNIST-Scale. MNIST digits are centered by default, and when placed in different positions to create MNIST-Position images, the viewpoint is easily distinguishable. For MNIST-Scale however, there is little visual variation between adjacent scales, which leads to a poor Top-1 classification accuracy for viewpoint (scale) classification.

As the main paper can only have 6 figures, we are unable to move \ref{fig:accuracy_tasks} to the main paper. However, we have cited this in the main paper along with the above discussion.

\textbf{R2: Explain in more detail what causes that the number of specialized neurons for one task is larger than for the other task.} 

In supplement~\ref{app:SpecializationAdditionalDatasets}, cited in the "When" section of the main paper, we have added the following:


We also observe that for a small number of in-distribution combinations, the ratio of neurons specialized for category or viewpoint classification may be impacted by the relative difficulty of these two tasks. We observe that when the accuracy is higher for category classification (shown in Fig.~\ref{fig:accuracy_tasks}), a higher fraction of neurons becomes specialized for category, as observed for the iLab and MNIST-scale datasets. Similarly, when accuracy for viewpoint classification is higher, a greater fraction of neurons becomes specialized for viewpoint, as observed in  MNIST-Position.



\textbf{R2: Comment on deformable objects and symmetries.} 

In supplement~\ref{sec:suplLimits}, cited in the conclusions in the main paper, we have added the following discussion:

In this paper we have only considered rigid objects, while general object recognition often involves deformable and articulated object categories including humans and other animals.For such objects, parts may appear in various configurations for the same viewpoint. One way to analyze this more complex scenario would be to extend our experiments to study combinations of configurations, viewpoints and categories. Furthermore, this analysis may also be extended to study the impact of object symmetries, which would alter the effective number of visually distinct object viewpoints.


==> sections/intro_short.tex <==
\section{Main}\label{sec:introduction}
Data can impact generalization behaviour. Data is so different for machines. Can we use this to improve behaviour?

The data is so different. It is well known the data impacts generalization behaviour. Here we investigate if blah blah, and if computer vision needs to move in this direction.

Generalization behaviour is so different. It is known that diet impacts behaviour. Can we improve behaviour with diet?

% Biological vision generalizes effortlessly across changes in the real world. Be it changes in lighting, layout and orientation of objects in a room, new upholstery on the sofa, or even new flooring---biological vision continues to work with ease. In contrast, visual recognition models are well known to fail at generalizing across such real-world transformations including unseen lighting~\cite{madan2021small,beery2018recognition, zhang2021adversarial}, 2D rotations and shifts~\cite{zhang2019making, chaman2021truly}, viewpoints~\cite{barbu2019objectnet, liu2018beyond, zeng2019adversarial, madan2021small}, and colors~\cite{joshi2019semantic,shamsabadi2020colorfool}, among others. The dominant narrative guiding modern approaches to alleviate this generalization gap has been to improve \textit{how} machines process the data provided to them, relying on large-scale, internet scraped datasets as benchmarks for generalization. This includes improving data pre-processing through data augmentation~\cite{} or generative modeling~\cite{}, extracting features better suited for generalization~\cite{}, and proposing specialized architectures optimized for domain generalization~\cite{}, among others. However, despite unprecedented progress, human-like generalization remains an unsolved problem~\cite{}.

% In this article, we present an alternative perspective on addressing this generalization gap inspired by behavioural neuroscience---instead of focusing on differences in \textit{how }data is processed, we focus on the fundamental differences in the data itself i.e. the visual diet of humans and machines. \textbf{MOTIVATE MORE}. 

% We highlight two major differences between the visual diet of biological and machine vision systems. Firstly, children learn from the physical space they occupy---a few $3$D scenes and objects while sampling densely from their surroundings under diverse real-world transformations. This includes viewing the same room from different viewpoints, under different lighting over the day, natural occlusions due to the room's layout, and sometimes even changes in object textures. Secondly, humans always view objects in the context of their surroundings. In contrast, popular internet scraped datasets like ImageNet~\cite{deng2009imagenet} and CIFAR~\cite{krizhevsky2009learning} contain sparsely sampled information ($\sim 1$ photograph) from a large number of $3$D scenes. Each image is a single snapshot into the information available in the original scene, and data augmentation methods like $2$D rotations and crops do not reflect the complex real-world transformations seen by the human visual system listed above. Furthermore, these images show objects with minimal scene context with most of the image occupied by a single objects placed in the center. For brevity, we refer to these as differences in \textit{transformational diversity} and \textit{scene context}, respectively. 

% In this article, we evaluate if mimicking these attributes of human-like visual diet can positively impact generalization behaviour of visual recognition models. These experiments are enabled by one new dataset which mimicks the human visual diet, and a new model which is designed to leverage this visual diet. Below we provide more details on these.

% Foreshadowing our results, a simple architecture with the right data far outperforms specialized approaches with data lacking these attributes. 

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/fig1.pdf}
    \caption{\textbf{Semantic Shifts in Context (\textit{SSIC}) Dataset:} (a) Natural image from the ScanNet dataset. (b) Paired photo-realistic image created by reconstructing object geometry, scene layout and camera parameters. (c) Image created by modifying the materials of the reconstructed image while holding viewpoint and light constant. (d) Image created by modifying the lighting of the reconstructed image while holding viewpoint and materials constant.(e) Image created by modifying the camera viewpoint of the reconstructed image while holding materials and light constant. Furthermore, target object (table) is always shown in the context of its surroundings.}
    \label{fig:teaser_figure}
\end{figure*}

% To alleviate this gap in visual diet, we introduce the new \textit{Human Visual Diet (HVD)} dataset, which models both transformational diversity and scene context to better mimick data seen by the human visual system. \textit{HVD} was created by 3D reconstructing scenes from ScanNet~\cite{} using the OpenRooms framework~\cite{}, and rendering new images from the reconstructed 3D scenes with controlled real-world transformations in scene lighting, object materials, and viewpoints. \textbf{Fig.~\ref{fig:teaser_figure}} shows a natural image from ScanNet, a paired photo-realistic image reconstructed using OpenRooms~\cite{li2020openrooms}, and one image each for lighting, material, and viewpoint variation introduced in \textit{HVD}. As can be seen, objects in \textit{HVD} are shown in context, and under disentangled, diverse real-world transformations.


% We introduce the novel dataset which mimicks the human visual diet---the \textit{Semantic Shifts in Context (SSIC)} dataset. \textit{SSIC} contains objects shown in context, and has systematic subsets with controlled, disentangled semantic shifts in scene lighting, viewpoint, and material. 

% Combined, these attributes enable mimicking the distribution of the data seen by humans, i.e., the human visual diet. \textit{SSIC} was created by reconstructing $1,288$ real-world 3D scanned scenes from the ScanNet dataset~\cite{} using the OpenRooms framework~\cite{li2020openrooms}, and rendering new images from these 3D scenes with \textit{transformational diversity} by introducing controlled variations in scene lighting, object materials, and viewpoints. \textbf{Fig.~\ref{fig:teaser_figure}} shows a real-world image from ScanNet, a paired photo-realistic image reconstructed using OpenRooms~\cite{li2020openrooms}, and one image each with disentangled semantic shifts in materials, lighting and viewpoint from our \textit{SSIC} dataset. As can be seen, objects (\eg table) are shown in context, and under disentangled, diverse real-world transformations in viewpoint, lighting and material. To replicate our analyses with natural images, we also modified the iLab dataset~\cite{borji2016ilab} to create the \textit{Semantic-iLab} dataset containing viewpoint, material and light shifts (Supplement \textbf{Sec.~\ref{supplsec:semantic_ilab_images}}). 
% Using these datasets, we quantified the impact of \textit{transformational diversity} on generalization.

% As existing recognition models are not designed to exploit scene context and transformational diversity, we also propose a new model to leverage the visual diet presented in \textit{HVD}---the Contextual Transformation Contrastive Net (CTCNet). Our model explicitly leverages scene context by using two separate streams to process the object and context independently before reasoning over them jointly. To exploit transformational diversity, CTCNet uses supervised contrastive loss across real-world transformations in lighting, viewpoint and materials (see Methods).

% To encourage CTCNet to learn robust and generic context information across domains, we apply supervised contrastive loss on the context-modulated object representations, which attracts the latent representations of the context where the target objects from the same object category are located, and repels the irrelevant context. By comparing the generalization behaviour of CTCNet against standard models not using scene context, we quantified the impact of using scene context on generalization.

% Building on these components, our experiments provide compelling evidence that modeling and mimicking the human-like visual diet enables substantially better generalization, and outperform by a large margin specialized architectures or data augmentation techniques trained without transformational diversity and scene context. Concretely, we introduce the following discoveries.

% % Firstly, our experiments show that both \textit{transformational diversity} and \textit{scene context} substantially improve generalization to out-of-distribution real-world transformations including lighting, viewpoints, and materials. Our first 

% Firstly, all architectures show a significant increase in performance as transformational diversity is increased. This is sufficient to generalize to OOD lighting. While it increases performance on OOD materials and viewpoint variations significantly, there is still room for further improvement. It is also observed that increasing diversity in one transformation does not lead to improved performance on a different transformation. Thus, performance gains do not transfer across real-world transformations.

% Secondly, training models which utilize both transformational diversity and scene context outperform specialized domain generalization approaches by a large margin---in some instances as high as 18\%. Furthermore, popular data-augmentation techniques like rotations and crops perform significantly worse than real-world transformations at enabling generalization. This is consistent with the finding of performance not transferring across transformations, as these data augmentation techniques do not capture the complexity of the real-world transformations.

% Thirdly, we observe that these findings can also be used to train models that generalize well to images from the real-world ScanNet~\cite{dai2017scannet} dataset, despite never being trained with natural images from this dataset. Mimicking human-like visual diet enables a 17\% margin in performance above state-of-the-art architectures and methods that do not leverage transformational diversity and scene context.
% % Finally, we also conduct psychophsyics experiments on \textit{SSIC} to quantify the generalization capabilities of human vision and establish an upper bound for future work.

% % Our key contributions include:
% %  \vspace{-2mm}
% % \begin{itemize}
% %     \itemsep-0.5em
% %     \item A new dataset (\textit{SSIC}) mimicking human visual diet with controlled, real-world semantic shifts (Lighting, Material and Viewpoints) and scene context. This amounts to $300,000$ images and over $1$ million object instances.
% %     \item A context-aware object recognition model, designed to leverage a human-like visual diet---CTCNet.
% %     % \item We present a controlled analysis of real-world transformations, showing that viewpoint shifts constitute a central challenge for existing models. While materials can be handled with data diversity, and lighting is very easy to generalize across.
% %     \item A new approach to reconcile the generalization gap between biological and computer vision---mimicking human visual diet, which improves generalization across semantic shifts in both synthetic and natural images.
% % \end{itemize}

% % Building on recent work using photo-realistic data to evaluate generalization behaviour \cite{leclerc20213db, madan2021small, madan2022and, bomatter2021pigs},

% % Building on existing approaches for domain generalization that increase data diversity and enforce consistency across diverse views~\cite{hendrycks2019augmix, zhang2017mixup, xu2020randconv}, we increase diversity by using multiple domains with disjoint sets of light settings, materials, and viewpoints.

==> sections/related_work.tex <==
% \section{Related Work}\label{sec:related_work}
% Below we present literature on existing approaches to improve generalization performance, and on visual diet.

% \subsection{Domain generalization approaches}


% \textbf{Approaches:} Existing solutions fall largely into three categories~\cite{zhou2021domain}---(1) Increasing data diversity through augmentation~\cite{zhang2017mixup, hendrycks2019augmix, xu2020randconv}, generative modeling~\cite{huang2017adain}, or adversarial approaches~\cite{xie2020adversarial, shankar2018generalizing, qiao2020learning, sinha2017certifying, NEURIPS2018_1d94108e}, (2) Enforcing invariance~\cite{arjovsky2019invariant, erfani2016robust, chattopadhyay2020learning, wang2021respecting, li2017deeper}, and (3) Modifying the learning strategy using meta-learning or ensemble learning~\cite{li2018learning, balaji2018metareg, zhou2021domain} Of these, approaches relying on increasing data diversity are the closest to our methodology. This includes data augmentation techniques like MixUp~\cite{zhang2017mixup}, AugMix~\cite{hendrycks2019augmix}, RANDConv~\cite{xu2020randconv}, style transfer based methods using AdaIN~\cite{huang2017adain}, and adversarial approaches to increase data diversity during training~\cite{xie2020adversarial, shankar2018generalizing, qiao2020learning, sinha2017certifying, NEURIPS2018_1d94108e}. However, unlike our approach these do not use scene context or increase diversity using lighting, material and viewpoint variations.
\looseness=-1

% \subsection{Generalizing to OOD image transformations}
% Beyond domain generalization, there is also significant work on generalizing across transformations like 2D rotations and shifts~\cite{zhang2019making, chaman2021truly}, and commonly occurring perturbations like blur or noise patterns~\cite{hendrycks2019benchmarking, mintun2021interaction, xie2020adversarial, xie2020self}. Some works have also investigated the robustness of visual recognition models to interpretable image transformations like changes in lighting~\cite{madan2021small,beery2018recognition, zhang2021adversarial}, viewpoints~\cite{barbu2019objectnet, liu2018beyond, zeng2019adversarial, madan2021small}, geometric modifications~\cite{belder2022random, xiao2019meshadv, yang2018realistic},  and even color changes~\cite{joshi2019semantic,shamsabadi2020colorfool}. Recently, the community has also explored generalization to more global, real-world transformations using photo-realistic synthetic data, which include---3D rotations~\cite{cooper2021out, sakai2021three}, OOD category-viewpoint combinations~\cite{madan2022and} and incongruent scene context~\cite{bomatter2021pigs,zhang2020putting}. Our work builds on these ideas, and investigates the impact of visual diet on enabling generalization across such real world transformations.

% \subsection{Visual diet of biological vs computer vision}
% \textbf{Impact of data on biological and computer vision:}
% For biological vision, there is a long history of works showing that changing the visual diet alters the visual cortex~\cite{kreiman2021biological, kandel2000principles}. There is rich developmental literature studying how biological vision is impacted by visual diets deprived of faces~\cite{arcaro2017seeing}, binocular vision~\cite{hubel1964effects}, environmental directionality~\cite{daw1976kittens}, and temporally smooth objects~\cite{wood2018development}, among several others. Some works have also tried to quantitatively define the human visual diet~\cite{clerkin2017real}. Recently, some computational works have also studied how the data distribution (visual diet) impacts visual search assymetries~\cite{gupta2021visual}, and object recognition~\cite{madan2022and,madan2021small}. Here, we build on these ideas to explore its impact on generalization across semantic shifts.

% \textbf{Role of context in vision:} There is a long history of work studying the role scene context in human vision~\cite{doi:10.1177/09567976211032676, greene2013statistics, graef1992scene, torralba2006contextual, henderson1992object, mathis1998does,zhang2020putting} and modelling contextual cues computationally~\cite{torralba2006contextual, taylor2013context,zhang2020putting,bomatter2021pigs}. Recently, some works have studied the impact of congruent and incongruent scene context on humans and computer vision~\cite{zhang2020putting, bomatter2021pigs}, and proposed an architecture to better generalize to incongruent scene contexts~\cite{bomatter2021pigs}. We build on these ideas and study the impact of context on generalization across semantic shifts.
